Object-based Illumination Estimation with Rendering-aware Neural Networks

We present a scheme for fast environment light estimation from the RGBD appearance of individual objects and their local image areas. Conventional inverse rendering is too computationally demanding for real-time applications, and the performance of purely learning-based techniques may be limited by the meager input data available from individual objects. To address these issues, we propose an approach that takes advantage of physical principles from inverse rendering to constrain the solution, while also utilizing neural networks to expedite the more computationally expensive portions of its processing, to increase robustness to noisy input data as well as to improve temporal and spatial stability. This results in a rendering-aware system that estimates the local illumination distribution at an object with high accuracy and in real time. With the estimated lighting, virtual objects can be rendered in AR scenarios with shading that is consistent to the real scene, leading to improved realism.

==> fig_comp.tex <==
%!TEX root = fastlightest.tex


\begin{figure*}
   \centering
\bgroup
\scriptsize
\renewcommand{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.2}
\begin{tabular}{m{1em} m{\fiveColumnFigWidth}m{\fiveColumnFigWidth}m{\fiveColumnFigWidth}m{\fiveColumnFigWidth}m{\fiveColumnFigWidth} c m{\fiveColumnFigWidth}m{\fiveColumnFigWidth}m{\fiveColumnFigWidth}m{\fiveColumnFigWidth}m{\fiveColumnFigWidth}}
& \multicolumn{1}{c}{Reference} & \multicolumn{1}{c}{Ours} & \multicolumn{1}{c}{Sato-Pred} & \multicolumn{1}{c}{Sato-GT} & \multicolumn{1}{c}{Gardner} & & \multicolumn{1}{c}{Reference} & \multicolumn{1}{c}{Ours} & \multicolumn{1}{c}{Sato-Pred} & \multicolumn{1}{c}{Sato-GT} & \multicolumn{1}{c}{Gardner}\\
%\vspace{0pt}\\
 \rotatebox{90}{Render}&
 %Case 75 in Specular Scene
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/render_gt.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/render_our.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/render_sato_pred.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/render_sato_gt.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/render_gard.png}& \hspace{2pt} &
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/render_gt.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/render_our.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/render_sato_pred.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/render_sato_gt.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/render_gard.png}\\
 \rotatebox{90}{Light}&
 %102 Single
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/light_gt.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/light_our.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/light_sato_pred.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/light_sato_gt.png} &
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/01/light_gard.png}& \hspace{2pt} &
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/light_gt.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/light_our.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/light_sato_pred.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/light_sato_gt.png}&
\includegraphics[width=\fiveColumnFigWidth]{fig/compare/02/light_gard.png}\\
\end{tabular}
\egroup
    %\vspace*{-0.4cm}
    \caption{Comparison to existing works. We compare our method to scene-based lighting estimation \cite{Gardner2017} (Gardner), and a classical inverse rendering method \cite{Sato2003IFS}. We test \cite{Sato2003IFS} with the shading map estimated by our decomposition (Sato-Pred) and with the ground truth shading map (Sato-GT) as well. }
    \label{fig:compare}
\end{figure*}

==> fig_layout.tex <==
%!TEX root = fastlightest.tex


\begin{figure}
   \centering
\bgroup
\small
\renewcommand{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.2}
\begin{tabular}{m{1em} m{\fourColumnFigWidth}m{\fourColumnFigWidth} c m{\fourColumnFigWidth}m{\fourColumnFigWidth}}
& \multicolumn{3}{c}{(a) Simple layout} & \multicolumn{2}{c}{(b) Complex layout}\\
%\vspace{0pt}\\
 \rotatebox{90}{Render}&
\includegraphics[width=\fourColumnFigWidth]{fig/layout_robustness/01/render_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/layout_robustness/01/render_pred.png}& \hspace{2pt} &
\includegraphics[width=\fourColumnFigWidth]{fig/layout_robustness/02/render_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/layout_robustness/02/render_pred.png}\\
 \rotatebox{90}{Light}&
\includegraphics[width=\fourColumnFigWidth]{fig/layout_robustness/01/light_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/layout_robustness/01/light_pred.png}& \hspace{2pt} &
\includegraphics[width=\fourColumnFigWidth]{fig/layout_robustness/02/light_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/layout_robustness/02/light_pred.png}\\
\end{tabular}
\egroup
    \vspace*{-0.2cm}
    \caption{Examples of (a) a simple layout with a few scattered objects, and (b) a complex layout with multiple objects in proximity, strong occlusions, and without a clear supporting surface.}
    \label{fig:layout_robustness}
\end{figure}

==> fig_light_size_num.tex <==
%!TEX root = fastlightest.tex


\begin{figure}
   \centering\includegraphics[width=0.48\textwidth]{fig/size_num_plot.png}
    \caption{Light estimation and re-rendering errors with respect to light source sizes and numbers. }
    \label{fig:size_number_plot}
\end{figure}

==> fig_local.tex <==
%!TEX root = fastlightest.tex


\begin{figure}
   \centering\includegraphics[width=0.9\textwidth]{fig/local/compose.png}
   \vspace*{-0.3cm}
    \caption{Spatially-varying illumination result by estimating light with different spatial crops from the input image (marked in blue). The virtually inserted toy planes exhibit shading consistent with the input, as the left plane casts shadow to the left, like the nearby pen stand, and the right plane casts shadow towards the right, similar to the nearby mug. Such spatially varying lighting effects are typical of near-field illumination. }
    \label{fig:local} 
\end{figure}

==> fig_material_robust.tex <==
%!TEX root = fastlightest.tex


\begin{figure*}
   \centering
\bgroup
\small
\renewcommand{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.2}
\begin{tabular}{m{1em} m{\fourColumnFigWidth}m{\fourColumnFigWidth} c m{\fourColumnFigWidth}m{\fourColumnFigWidth} c m{\fourColumnFigWidth}m{\fourColumnFigWidth}  c m{\fourColumnFigWidth}m{\fourColumnFigWidth}}
& \multicolumn{3}{c}{(a) $\rho_s=0.5, \rho_d=0.5, \sigma=0.01$} & \multicolumn{3}{c}{(b) $\rho_s=0.5, \rho_d=0.5, \sigma=0.1$} & \multicolumn{3}{c}{(c) $\rho_s=1.0, \rho_d=0.0, \sigma=0.1$} & \multicolumn{2}{c}{(d) $\rho_s=1.0, \rho_d=0.0, \sigma=0.1$}\\
%\vspace{0pt}\\
 \rotatebox{90}{Render}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/01/render_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/01/render_pred.png}& \hspace{2pt} &
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/02/render_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/02/render_pred.png}& \hspace{2pt} &
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/03/render_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/03/render_pred.png}& \hspace{2pt} &
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/04/render_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/04/render_pred.png}\\
 \rotatebox{90}{Light}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/01/light_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/01/light_pred.png}& \hspace{2pt} &
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/02/light_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/02/light_pred.png}& \hspace{2pt} &
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/03/light_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/03/light_pred.png}& \hspace{2pt} &
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/04/light_gt.png}&
\includegraphics[width=\fourColumnFigWidth]{fig/material_robustness/04/light_pred.png}\\
\end{tabular}
\egroup
    \vspace*{-0.4cm}
    \caption{Lighting estimation and re-rendering results for objects with different materials, including (a) highly specular, (b) glossy, (c) predominantly diffuse, and (d) purely diffuse.}
    \label{fig:material_robustness}
\end{figure*}

==> fig_real_comp.tex <==
%!TEX root = fastlightest.tex
\newcommand{\RealGTInputSize}{0.05}
\newcommand{\RealGTRenderSize}{0.05}
\newcommand{\RealGTCubeSize}{0.05}

\newcommand{\GTCompLayout}[1]{

        \begin{minipage}[c] {\RealGTInputSize\textwidth}
            \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/real/#1/rgb.png}
            %\vspace*{-0.8cm}\caption*{Input RGB}
            \end{minipage}
            \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/real/#1/depth.png}
            %\vspace*{-0.8cm}\caption*{Input Depth}
            \end{minipage}
        \end{minipage}
        %\hspace*{0.7cm}
        \begin{minipage}[c] {\RealGTRenderSize\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/real/#1/Result_Pred.png}
            %\vspace*{-0.8cm}\caption*{Our result}
        \end{minipage}
        \begin{minipage}[c] {\RealGTRenderSize\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/real/#1/Result_GT.png}
            %\vspace*{-0.8cm}\caption*{Reference}
        \end{minipage}
        %\hspace*{0.7cm}
        \begin{minipage}[c] {\RealGTCubeSize\textwidth}
            \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/real/#1/Result_Pred_light_view.png}
            %\vspace*{-0.8cm}\caption*{Our result}
            \end{minipage}
            \begin{minipage}[t]{\textwidth}
            \centering
            \includegraphics[width=\textwidth]{fig/real/#1/Result_GT_light_view.png}
            %\vspace*{-0.8cm}\caption*{Reference}
            \end{minipage}
        \end{minipage}
}
\begin{figure}
    %\centering
    %\GTCompLayout{06}\GTCompLayout{05}
    \includegraphics[width=0.48\textwidth]{fig/real/fig_real.png}
\vspace*{-0.02cm}
    \caption{Real capture examples with comparison to measured ground truth lighting.
    We compare the estimated environment map against measured ground truth,
    as well as results rendered with our lighting and ground truth lighting.
    Please refer to the input RGB image to determine which object is virtually inserted.
    }
    \label{fig:realgt}
\end{figure}

==> fig_rgbonly.tex <==
%!TEX root = fastlightest.tex

\newcommand{\figWdightRGBOnly}{3cm}
\begin{figure}
   \centering
\bgroup
\small
\renewcommand{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.2}
\begin{tabular}{m{\figWdightRGBOnly} m{\figWdightRGBOnly}m{\figWdightRGBOnly}}

%\vspace{0pt}\\
\includegraphics[width=\figWdightRGBOnly]{fig/rgbonly/input.png}&
\includegraphics[width=\figWdightRGBOnly]{fig/rgbonly/ours.png}& 
\includegraphics[width=\figWdightRGBOnly]{fig/rgbonly/gt.png}\\
\multicolumn{1}{c}{Input} & \multicolumn{1}{c}{Our result} & \multicolumn{1}{c}{Reference}
\end{tabular}
\egroup
    \vspace*{-0.4cm}
    \caption{Lighting estimation with only RGB input, the depth is estimated by a separated nerual network then acts as our input.}
    \label{fig:rgbonly}
\end{figure}

==> tab_ablation.tex <==
%!TEX root = fastlightest.tex

\begin{table}[t!]
\begin{center}
%\begin{minipage}[t]{0.45\textwidth}
\centering
\begin{tabular}{ l | c c }
	& Render & Light \\
\hline
\multicolumn{3}{c}{Comparasion}\\
\hline
\cite{Gardner2017} & 0.133 & 3.056 \\
\cite{Sato2003IFS} + our decomposition & 0.098 & 1.851 \\
\cite{Sato2003IFS} + ground truth shading & 0.090 & 1.944 \\
\hline
\multicolumn{3}{c}{Ablation}\\
\hline
Diffuse only         & 0.076		& 1.447 \\
Specualr only  		 &0.081		& 1.440 \\
Without decomposition& 0.074		& 1.434 \\
Direct regression	 & 0.072		& 1.432 \\
\hline
Our results  & 0.069 &  1.429 \\
Our results (+recurrent layer)	 & \textbf{0.068}	& \textbf{1.419}\\
Our results (estimated depth)	 & 0.078	& 1.437\\
    \hline
  \end{tabular}
\caption{Average RMSE of estimated lights and rerender images.   }
\label{tab:ablation}
%\end{minipage}
\end{center}
\end{table}
